Trial by Flyer: Building Quadcopters From Scratch in a Ten-Week Capstone Course

We describe our experience teaching an intensive capstone course in which pairs of students build the hardware and software for a remote-controller quad-rotor aircraft (i.e., a quadcopter or "drone") from scratch in one 10-week quarter. The course covers printed circuit board (PCB) design and assembly, basic control theory and sensor fusion, and embedded systems programming. To reduce the workload on course staff and provide higher-quality feedback on student designs, we have implemented an automated PCB design checking tool/autograder. We describe the course content in detail, identify the challenges it presents to students and course staff, and propose changes to further increase student success and improve the scalability of the course.

==> background.tex <==
\section{Course Overview}
\label{sec:background}



==> design.tex <==
\section{Tuning the Class}





\subsection{Costs}

A frequent complaint about the course is that the students are not able to
continue working on their \qs{} after the course ends.  The reason for this
is that the remote control design we have used is expensive -- \~\$200.  The
\qs{} are also moderately expensive -- \fixme{\~\$50}.  In addition, for the
\q{} to useful, they also need one or more batteries, a battery charger, and a
small programming board.

Our goal is to let each student take home a working remote, one of their \qs{},
and all the necessary equipment for under \~\$100 -- the cost of a high-end
text book.

To achieve this we have built a bare-bones remote that dispenses with some
useful, but expensive features like an on-board LCD for displaying status
information (\$25).  We also added one feature to make the system usable after
the course and makes it easier for students to work outside the classroom: The
remote has a built-in LiPo battery charger.

We have also started purchasing motors and electrical components in bulk, which
can reduce costs for those parts by up between \fixme{\$X} and \fixme{\$Y}.

During the next iteration of the class, we expect to have the per-student cost
down to \~\$\fixme{130}, a significant improvement but still more expensive
than we would like.  Long term, we are looking at using Bluetooth and replacing
remotes with an app on students' smartphones.

\ignore{

We are working to optimize the cost of each component:

\boldparagraph{\Q{}} The PCB itself accounts for \fixme{X}\% of \q{}'s cost.
We buy five (the minimum) copies of each board from the board manufacturer for
(on average) \fixme{\$X}/board.

There are several ways to decrease the cost of the boards.  First, we can
purchase components in bulk.  In past years, each student purchased a spare
parts kit for a commercially available quadcopter that included the motors,
propellers, and batteries for \$20.  Buying these components in bulk will
reduce the cost to \$\fixme{x}/student.  The downside is that we need to
purchase parts for many students (\~50) at a time.

Second, we could increase group size from two to three.  Since we have to buy
five boards, we could reduce the cost per student by having more students share
a design.  The downside is increased group size, which means individual
students will miss out on more aspects of the design process.

Finally, we limit the size of the boards and color.  Currently, the PCB's
include the ``arm,'' which increases the size of the boards significantly.
Instead, we could restrict the boards to \fixme{50\mm{}\x{}\50\mm{}} and use a
laser cutter to provide ``arms.''  This would reduce the cost of each board by
\fixme{X}\$.  Restricting boards to be green will save \fixme{x}\$/board.

Students are not in favor of larger group sizes or smaller, more restricted
board design.

\boldparagraph{Remote Control} Our original remote design was badly
over-designed, so most of the savings came shrinking and simplifying the design.
We did make one significant sacrifice, however.  We removed the 16\x{}2 character
LCD screen that students used to display status information and to tune the
parameters of the PID controllers.  It was useful but cost \$25.

We also added an integrated battery charger, so the students can charge their
own battery during the class and after.

\boldparagraph{Other Equipment} To program the \q{} and the remote, the
students need a FTDI programming board.  These cost \$15, and we loan them to
students for the length of the course. 

  

To address this, we have redesigned the remote control to reduce its cost
significantly.}


\subsection{Quadcopter Design}

The details of the \q{} design have been very stable across the last three
iterations of the class.  The design is optimized for simplicity, reliability,
and ease of assembly.

All told, the \q{} PCB just \fixme{X} components, and the component count has
drop slightly year to year as we remove parts that are not necessary.  Where
possible, we select physically larger components that easier to place and
solder correctly.  These account for \fixme{X} of the parts.

\cfigure[Figures/NarrowMissing.pdf,{\figtitle{Package Types} Most of the parts
    are (relatively) large ``0805'' parts (left)).  The balun, voltage
    regulator, IMU, and microcontroller have finely-space connections.  The IMU
    is the most challenging because its ``pins'' are completely underneath the
    device.},fig:parts]

The remainder include the microcontroller, the IMU, the voltage regulator, and
a balun (a specialized component that is part of the antenna driver circuit).
These parts are more challenging because they small, closely-spaced electrical
connections \reffig{fig:parts}.  These are more representative of the
components modern electronics are built from.

The IMU is, by far, the most problematic part because its ``pins'' are
underneath the device, so there is no way to touch up the soldering job if it
goes wrong.  In the most recent iteration of the class the success rate for
soldering the IMU was just \fixme{x}\%, and repeated attempts consumed an
enormous amount of student and course staff time.  We are working hard to
debug this problem.

Changing IMUs is one alternative.  The microcontroller has a similar package
but its pins are exposed, albeit just barely.  This difference has a huge
impact in student success -- the failure rate was near zero.  Unfortunately,
there is no high-quality IMU with both a gyroscope and an accelerometer in a
similar package.  There are, however, separate gyroscope and accelerometers
packaged in that way.



==> grading.tex <==
\section{Evaluation}

\subsection{Grading Scheme}

\subsection{Measuring Success}

Success rate

\subsection{Observations}

CSE students do the worst, learn the most.


==> impl.tex <==
\section{System}
\label{sec:system}


==> labs.tex <==
\section{The Schedule}
\label{sec:labs}

The biggest challenge in teaching the course is the quarter system.  Packing
everything into ten weeks has driven changes in all aspects of the course,
including the design of the hardware we build.


\reffig{fig:schedule} shows the schedule of the course.  The course includes
\fixme{eleven} labs divided into two tracks: hardware and software.  The course
meets twice a week for ninety-minute lecture followed immediately by a
ninety-minute lab.

Designing, manufacturing, and assembling the PCB form the critical path to a
working \q{}, and the first half of the class focuses primarily on bringing the
students up to speed quickly on the PCB design tools, PCB design concepts, the
\q{} design they are building, and the parts they will use.





There are three key challenges in the class: Designing the PCB, implementing
the flight control software, and assembling the PCB.

During the first five weeks of the class, the top priority is completing their
\q{} designs so we can get boards manufactured as soon as possible.  This
maximizes the time they have to assemble, test, and program their \qs{}.

In the best case, students start assembling their \q{} PCBs in \week{7},
leaving just four weeks to complete their project. 


The labs are staggered 





==> libpaper/arxiv.tex <==

\usepackage{fancyhdr}
\pagestyle{fancy}

\fancyhead{} %
\renewcommand{\headrulewidth}{0pt} %
\fancyfoot{} %

\fancyfoot[LE,RO]{\thepage}           %
\fancyfoot[RE,LO]{\scriptsize Copyright \textcopyright~\the\year\ the authors.\\{\tiny \gitcommit}} %


==> libpaper_metadata.tex <==
\newcommand{\gitcommit}{Uncommitted changes}
\def\arxivbuild{}


==> related.tex <==
\section{Related Work}
\label{sec:related}

